An Algebraic Framework for Compositional Program Analysis

The purpose of a program analysis is to compute an abstract meaning for a program which approximates its dynamic behaviour. A compositional program analysis accomplishes this task with a divide-and-conquer strategy: the meaning of a program is computed by dividing it into sub-programs, computing their meaning, and then combining the results. Compositional program analyses are desirable because they can yield scalable (and easily parallelizable) program analyses. This paper presents algebraic framework for designing, implementing, and proving the correctness of compositional program analyses. A program analysis in our framework defined by an algebraic structure equipped with sequencing, choice, and iteration operations. From the analysis design perspective, a particularly interesting consequence of this is that the meaning of a loop is computed by applying the iteration operator to the loop body. This style of compositional loop analysis can yield interesting ways of computing loop invariants that cannot be defined iteratively. We identify a class of algorithms, the so-called path-expression algorithms [Tarjan1981,Scholz2007], which can be used to efficiently implement analyses in our framework. Lastly, we develop a theory for proving the correctness of an analysis by establishing an approximation relationship between an algebra defining a concrete semantics and an algebra defining an analysis.

==> coincidence.tex <==
 \section{Coincidence} \label{sec:coincidence}
 We now consider the question of when the algorithm presented in
 Section~\ref{sec:inter_analysis} computes the ideal (join-over-paths)
 solution to an analysis problem.  This is analogous to the development of
 \emph{coincidence theorems} \cite{Kam1977,Sharir1981,Knoop1992b,Lal2005} in
 the field of dataflow analysis, which state conditions under which the
 iterative algorithm for solving dataflow analyses computes the ideal
 solutions (i.e., when the join-over-paths solution to a dataflow analysis
 problem coincides with the minimum fixpoint solution\footnote{In dataflow
   analysis literature, coincidence theorems typically relate the
   meet-over-paths and the maximum fixpoint solutions.  We follow in the
   tradition of abstract interpretation, which uses the dual order.}).  In this
 section, we formulate and prove a coincidence theorem for our interprocedural
 framework.

 The first step towards formulating our coincidence theorem is to define the
 join-over-paths solution to an analysis.  This requires us to define what a
 path is, and how to interpret it.  Our treatment of interprocedural paths in
 Section~\ref{sec:inter_analysis} is not adequate for this purpose, because it
 relies on interpreting call edges using procedure summaries (which represent
 a set of paths, rather than a single path).  In this section, we will take
 interprocedural paths to be words over an alphabet of control flow graph
 edges such that each return is properly matched with a call.  For a formal
 definition of such a path, the reader may consult \cite{Sharir1981}.  We use
 \textsf{IPaths(v)} to denote the set of all interprocedural paths to $v$.

 Now we must define the interpretation of an interprocedural path.  Let
 $\mathscr{I} = \langle \mathcal{D}, \sem{\cdot} \rangle$ be an
 interpretation.  We define the interpretation of a path within $\mathscr{I}$
 as a function that operates on \emph{stacks} of abstract values (as in
 \cite{Knoop1992b,Lal2005}).  We use the notation $[\langle V_1, a_1 \rangle,
   \ldots, \langle V_n, a_n \rangle]$ to denote a stack of $n$
 \emph{activation records}, where an activation record is a tuple $\langle
 V_i, a_i \rangle$ consisting of a set of variables $V_i$ that are local to
 that activation record, and an abstract value $a_i$.  The first entry in this
 list corresponds to the top of the stack.  We define our semantic function on
 edges so that each call edge corresponds to a push on this stack, each return
 edge corresponds to a pop, and each intraprocedural edge modifies the top of
 the stack (i.e., the ``current'' activation record).  Formally, we have

 \vspace*{3pt}
 \noindent $\widehat{\sem{e}}([\langle V_1, a_1 \rangle, \ldots, \langle V_n, a_n \rangle]) =$\\
 \hspace*{0pt}\hfill$\begin{cases}
     [\langle LV_i, 1 \rangle,\langle V_1, a_1 \rangle,\ldots,\langle V_n, a_n \rangle] & \text{if } \act(e) = \texttt{call } i\\
     [\langle V_2, a_2 \mul (\exists V_1.a_1) \rangle, \ldots, \langle V_n, a_n \rangle] & \text{if } \act(e) = \texttt{return}\\
     [\langle V_1, a_1 \mul \sem{e} \rangle, \ldots, \langle V_n, a_n \rangle] & \text{otherwise}
   \end{cases}$
 \vspace*{3pt}

   We may then associate with every path $\pi$ a stack of activation records
   $S(\pi)$ in the following way:
   \begin{eqnarray*}
     \textit{stack}(\epsilon) &=& [\langle LV_1, 1 \rangle]\\
     \textit{stack}(\pi a) &=& \widehat{\sem{a}}(\textit{stack}(\pi))
   \end{eqnarray*}

   Next, we define a $\textit{flatten}$ function that lowers a stack of
   activation records into a single abstract value, and existentially
   quantifies variables that are not in the scope of the current activation
   record.
   \[\textit{flatten}([\langle V_1, a_1 \rangle, \ldots, \langle V_n,
     a_n \rangle]) = (\exists V_n. a_n)\mul \dotsi \mul (\exists V_2. a_2)
   \mul a_1\]

   Finally, we take the interpretation of an interprocedural path within
   $\mathscr{I}$ to be $\textit{flatten}(\textit{stack}(\pi))$.

   \subsection{Quantales}
   The next step in formulating our coincidence theorem is to define a
   condition under which we can guarantee that $\mathscr{I}\langle v \rangle$
   coincides with the join of $\textit{flatten}(\textit{stack}(\pi))$ over all
   paths $\pi$ ending at $v$.  For traditional dataflow analysis frameworks,
   the coincidence theorem holds for analyses where all transfer functions are
   distributive.  In our context, coincidence holds when the semantic algebra
   forms a (quantified) quantale \cite{Mulvey1986}.

   \begin{definition}[Quantale]
     A \emph{(quantified) quantale} is a tuple $\mathcal{Q} = \langle Q,
     \plus, \mul, \closure, \exists, 0, 1 \rangle$ such that $\mathcal{Q} =
     \langle Q, \plus, \mul, \closure, 0, 1 \rangle$ is a Kleene algebra, $Q$
     forms a complete lattice (under the natural order $\leq$), and such that
     $\mul$ and $\exists$ distribute over arbitrary sums.  That is, (for any
     index set $I$)
     \begin{align*}
       a\mul\big(\bigoplus_{i \in I} b_i\big) &= \bigoplus_{i \in I} (a\mul
       b_i)\\
       \big(\bigoplus_{i \in I} a_i\big)\mul b &= \bigoplus_{i \in I} (a_i\mul b)\\
       \exists x. \bigoplus_{i \in I} a_i &= \bigoplus_{i \in I} (\exists x. a_i)
     \end{align*}
   \end{definition}
   
   The standard definition of quantales omits the iteration operator and the
   quantification operator.  The introduction of the iteration operator loses
   no generality, because in any quantale the iteration operator may be
   defined uniquely as $a^\closure = \bigoplus_{n \in \mathbb{N}} a^n$.  The
   quantification is needed only for our interprocedural coincidence theorem,
   and may be omitted for the intraprocedural variant.

   Recalling the definition of $\mathscr{I}\langle v \rangle$ from
   Section~\ref{sec:inter_analysis}, we may state our coincidence theorem:
   \begin{theorem}[Coincidence] \label{thm:coincidence}
     Let $\mathscr{I} = \langle \mathcal{Q}, \sem{\cdot} \rangle$ be an
     interpretation, where $\mathcal{Q}$ is a quantale.  Then for any $v$,
     \begin{equation*}
       \mathscr{I}\langle v \rangle = \bigoplus_{\pi \in \mathsf{IPaths}(v)} \textit{flatten}(\textit{stack}(\pi))
     \end{equation*}
   \end{theorem}
   \begin{proof}
     The proof proceeds in two steps.  First, we define a \emph{quantified
       word} interpretation $\mathscr{W} = \tuple{\mathcal{W},
       \sem{\cdot}_{\mathcal{W}}}$, for which we can show a coincidence
     result.  Then, we show that any interpretation $\mathscr{I} =
     \tuple{\mathcal{Q}, \sem{\cdot}_{\mathcal{Q}}}$ over a quantale
     ``factors'' through the quantified word interpretation, in the sense that
     there is a quantale homomorphism $h$ such that
     \[\mathscr{I}\tuple{v} =
     h(\mathscr{W}\tuple{v})\]

     We first define the set of quantified words $W$ to be the empty word or
     any word recognized by the following context free grammar:
     \begin{align*}
       W ::= & e & e \in E\\
       | & (\exists x. W) & x \in \Var\\
       | & W W
     \end{align*}
     We then define a (weak) quantale
     \[ \mathcal{W} = \tuple{\powerset{W}, \cup, \mul_{\mathcal{W}}, \star_{\mathcal{W}}, \exists_{\mathcal{W}}, \emptyset, \{\epsilon\}} \]
     where
     \begin{align*}
       P\mul_{\mathcal{W}} Q &= \{ ab : a \in P, b \in Q \}\\
       P^{\star_{\mathcal{W}}} &= \bigcup_{n \in \mathbb{N}} P^n\\
         \exists x. P &= \{ (\exists x. a) : a \in P \}
     \end{align*}
     Note that $\mathcal{W}$ does not satisfy axioms (Q2)-(Q4).  It is for
     this reason that we call $\mathcal{W}$ a weak quantale.  However, the
     axioms (Q2)-(Q4) are irrelevant for this proof.

     We define the quantified word interpretation as $\mathscr{W} =
     \tuple{\mathcal{W}, \sem{\cdot}_{\mathcal{W}}}$, where
     $\sem{e}_{\mathcal{W}}$ is defined as the word consisting of a single
     letter $e$.

     Next, we define a function $h : \mathcal{W} \rightarrow \mathcal{Q}$ by
     \[ h(P) = \bigoplus_{\mathcal{Q}} \{ \tilde{h}(a) : a \in P \} \]
     where
     \begin{align*}
       \tilde{h}(e) &= \sem{e}_{\mathcal{Q}}\\
       \tilde{h}(ab) &= \tilde{h}(a) \mul_{\mathcal{Q}} \tilde{h}(b)\\
       \tilde{h}(\exists x.a) &= \exists_{\mathcal{Q}} x. \tilde{h}(a)
     \end{align*}

     We will use the subscripts $\mathcal{Q}$ and $\mathcal{W}$ on
     $\textit{stack}$ and $\textit{flatten}$ to distinguish between which
     interpretation it is being applied in.

     \begin{lemma} \label{lem:flatten}
       For any interprocedural path $\pi$,
       \[h(\textit{flatten}_{\mathcal{W}}(\textit{stack}_{\mathcal{W}}(\pi))) = 
       \textit{flatten}_{\mathcal{Q}}(\textit{stack}_{\mathcal{Q}}(\pi)) \]
     \end{lemma}
     \begin{proof}
       By induction on $\pi$.
     \end{proof}

     \begin{lemma} \label{lem:factor}
       For any $v$,
       \[ \mathscr{I}\tuple{v} = h(\mathscr{W}\tuple{v}) \]
     \end{lemma}
     \begin{proof}
       Define a relation $\soundrel \subseteq \mathcal{W} \times \mathcal{Q}$ as
       the graph of the function $h$.  That is,
       \[ \soundrel = \{ \tuple{P,h(P)} : P \in \mathcal{W} \} \]
       It is easy to show that $\soundrel$ is coherent w.r.t. the \QPKA{}
       operations.

       Next, we must show that for any $i$,
       $\sound{\overline{S}_{\mathcal{W}}(i)}{\overline{S}_{\mathcal{Q}}(i)}$.
       We may prove this by induction on the transfinite iteration
       sequence defining $\overline{S}_{\mathcal{W}}$ and
       $\overline{S}_{\mathcal{Q}}$ (using Lemma~\ref{lem:pathexp_rel} for the
       induction step).

       Finally, we may apply Lemma~\ref{lem:analysis_rel} to get
       \[ \sound{\mathscr{W}\tuple{v}}{\mathscr{I}\tuple{v}} \]
       whence $\mathscr{I}\tuple{v} = h(\mathscr{W}\tuple{v})$.
     \end{proof}

     It is easy to see that $\mathscr{W}\tuple{v}$ is exactly the set of
     interprocedural paths to $v$, where calls and returns have been replaced
     by existential quantification of the appropriate variables.  This can be
     expressed formally as
     \[w \in \mathscr{W}\tuple{v} \iff \exists \pi \in \mathsf{IPaths}(v). \{w\} = \textit{flatten}_{\mathcal{W}}(\textit{stack}_{\mathcal{W}}(\pi))\]
     Or equivalently, as
     \[ \mathscr{W}\tuple{v} = \bigcup_{\pi \in \mathsf{IPaths}(v)} \textit{flatten}_{\mathcal{W}}(\textit{stack}_{\mathcal{W}}(\pi)) \]

     We may then conclude
     \begin{align*}
      \mathscr{W}\tuple{v} &= \bigcup_{\pi \in \mathsf{IPaths}(v)} \textit{flatten}_{\mathcal{W}}(\textit{stack}_{\mathcal{W}}(\pi))\\
      h(\mathscr{W}\tuple{v}) &= h\Big(\bigcup_{\pi \in \mathsf{IPaths}(v)} \textit{flatten}_{\mathcal{W}}(\textit{stack}_{\mathcal{W}}(\pi))\Big)\\
      \mathscr{I}\tuple{v} &= h\Big(\bigcup_{\pi \in \mathsf{IPaths}(v)} \textit{flatten}_{\mathcal{W}}(\textit{stack}_{\mathcal{W}}(\pi))\Big) & \text{Lemma~\ref{lem:factor}}\\
      \mathscr{I}\tuple{v} &= \bigoplus_{\pi \in \mathsf{IPaths}(v)} h(\textit{flatten}_{\mathcal{W}}(\textit{stack}_{\mathcal{W}}(\pi))) & \text{Def'n of } h\\
      \mathscr{I}\tuple{v} &= \bigoplus_{\pi \in \mathsf{IPaths}(v)} \textit{flatten}_{\mathcal{Q}}(\textit{stack}_{\mathcal{Q}}(\pi)) & \text{Lemma~\ref{lem:flatten}}
     \end{align*}
   \end{proof}

 %% \begin{example}
 %%   It is easy to check that the domain for reaching definitions analysis forms
 %%   a quantale, because any finite \KA{} is a quantale.  It follows from our
 %%   coincidence theorem that the solution to the reaching definitions problem
 %%   computed by the path-expression algorithm coincides with the join over
 %%   paths solution.
 %% \end{example}

 %% \begin{proof}
 %%   Most of the quantale properties are easy to prove.  The only difficult case
 %%   is proving that function composition distributes over arbitrary joins.

 %%   Let $f \in D_L$, and let $\{ g_\alpha \}_{\alpha < \kappa}$ be a subset
 %%   of $D_L$ (indexed by some ordinal $\kappa$).  We need to prove that
 %%   \begin{equation*}
 %%     f \circ (\bigoplus_{\alpha < \kappa} g_\alpha) = \bigoplus_{\alpha <
 %%       \kappa} (f \circ g_\alpha)
 %%   \end{equation*}
 %%   Let $x \in L$.  Then $(f \circ (\bigoplus_{\alpha < \kappa} g_\alpha))(x)
 %%   = f((\bigoplus_{\alpha < \kappa} g_\alpha)(x)) = f(\bigoplus_{\alpha <
 %%     \kappa} g_\alpha(x))$.  Define a set $I \subseteq \kappa$ by
 %%   \begin{equation*}
 %%     I = \{ \alpha \in \kappa : \bigoplus_{\beta < \alpha} g_\beta(x) \neq \bigoplus_{\beta \leq \alpha} g_\beta(x) \}
 %%   \end{equation*}

 %%   It follows from the fact that $L$ satisfies the ascending chain condition
 %%   that $I$ is finite, since we can define a strictly ascending chain $\{
 %%   c_\alpha \}_{\alpha \in I}$ by taking
 %%   \begin{equation*}
 %%     c_\alpha = \bigoplus_{\beta \leq \alpha} g_\beta(x)
 %%   \end{equation*}

 %%   It is easy to check that $\bigoplus_{\beta < \alpha} g_\beta(x) =
 %%   \bigoplus_{\beta \in I} g_\beta(x)$.  Since $f$ distributes over finite
 %%   joins, we have
 %%   \begin{eqnarray*}
 %%     f(\bigoplus_{\alpha < \kappa} g_\alpha(x)) &=& f(\bigoplus_{\alpha \in I} g_\alpha(x))\\
 %%     &=& \bigoplus_{\alpha \in I} f(g_\alpha(x))\\
 %%     &\leq& \bigoplus_{\alpha < \kappa} f(g_\alpha(x))\\
 %%   \end{eqnarray*}
 %%   The other direction of the inequality follows from the fact that $f$ is
 %%   monotone.  So we may conclude that $f$ left-distributes over arbitrary
 %%   joins.  Proving that $f$ right-distributes over arbitrary joins is trivial.
 %% \end{proof}





==> inter_abstract.tex <==
 \section{Interprocedural Abstraction} \label{sec:inter_abstract}

 In this section, we adapt the abstract interpretation framework of
 Section~\ref{sec:intra_abstract} to the interprocedural setting presented in
 Sections~\ref{sec:interproc} and \ref{sec:inter_analysis}.  The conditions of
 Proposition~\ref{prop:ka_sr} are much easier to adapt to the interprocedural
 setting than the more general definition of a soundness relation, so we
 present this simplified version here.  Under the assumptions of
 Proposition~\ref{prop:ka_sr}, all that is required to extend soundness
 relations to the interprocedural setting is an additional coherence
 condition regarding the quantification operator.
 
 \begin{definition}[Interprocedural soundness relation]
   Let $\mathcal{C}$ be a quantified quantale and let $\mathcal{A}$ be a
   \QPKA{}.  A relation $\soundrel \subseteq \mathcal{C} \times \mathcal{A}$
   is a \emph{soundness relation} if $\soundrel$ satisfies the conditions of
   Proposition~\ref{prop:ka_sr}, and for all $\sound{c}{a}$, and all $x \in
   \Var$, we have $\sound{\exists_{\mathcal{C}} x. c}{\exists_{\mathcal{A}}
     x. a}$.
 \end{definition}

 The sound abstraction theorem carries over to the interprocedural setting,
 and is stated below.  The proof of this theorem (presented in the full
 version \cite{fullversion}) is more complicated than the intraprocedural
 variant, and requires the fixpoint machinery of classical abstract
 interpretation \cite{Cousot1977} due to the inductive summary assignment
 computation.

 \begin{theorem}[Sound abstraction] \label{thm:sound_abstraction}
   Let $\mathscr{C}, \mathscr{A}$ be interpretations, where the 
   domain of $\mathscr{C}$ is a quantified quantale and the domain of
   $\mathscr{A}$ is a \QPKA{}.  Let $\soundrel \subseteq \mathcal{C} \times
   \mathcal{A}$ be a soundness relation, and let $v$ be a vertex of some
   procedure.  If for all $e \in E$, $\sound{\natsem{e}}{\abssem{e}}$, then
   $\sound{\mathscr{C}\langle v \rangle}{\mathscr{A}\langle v \rangle}$.
 \end{theorem}

 %% \begin{proof}
 %%   We begin with two general lemmas concerning interprocedural
 %%   interpretations.  The main result is then a simple application of these two
 %%   lemmas.
 %%   \begin{lemma} \label{lem:pathexp_rel}
 %%     Let $\mathscr{I} = \tuple{\mathcal{I}, \sem{\cdot}_{\mathcal{I}}}$ and
 %%     $\mathscr{J} = \tuple{\mathcal{J},\sem{\cdot}_{\mathcal{J}}}$ be \QPKA{}
 %%     interpretations, let $S_{\mathcal{I}}$ and $S_{\mathcal{J}}$ be summary
 %%     assignments, and let $\soundrel \subseteq \mathcal{I} \times \mathcal{J}$ be
 %%     any relation that is coherent with respect to the \QPKA{} operators and
 %%     such that for all $e \in E$, 
 %%     \[ \sound{\mathscr{I}(S_{\mathcal{I}})[e]}{\mathscr{J}(S_\mathcal{J})[e]} \]
 %%     Then for any path expression $p$,
 %%     \[ \sound{\mathscr{I}(S_{\mathcal{I}})[p]}{\mathscr{J}(S_\mathcal{J})[p]} \]

 %%     Moreover, this holds even if $\mathcal{I}$ and $\mathcal{J}$ do not
 %%     satisfy any of the \QPKA{} axioms.
 %%   \end{lemma}
 %%   \begin{proof}
 %%     By induction on $p$.
 %%   \end{proof}
 %%   \begin{lemma} \label{lem:analysis_rel}
 %%     Let $\mathscr{I} = \tuple{\mathcal{I}, \sem{\cdot}_{\mathcal{I}}}$ and
 %%     $\mathscr{J} = \tuple{\mathcal{J},\sem{\cdot}_{\mathcal{J}}}$ be \QPKA{}
 %%     interpretations, and let $\soundrel \subseteq \mathcal{I}
 %%     \times \mathcal{J}$ be any relation that is coherent with respect to the
 %%     \QPKA{} operators and such that for all $e \in E$,
 %%     \[ \sound{\mathscr{I}(\overline{S}_{\mathcal{I}})[e]}{\mathscr{J}(\overline{S}_\mathcal{J})[e]} \]
 %%     where $\overline{S}_{\mathcal{I}}$ and $\overline{S}_{\mathcal{J}}$ are
 %%     inductive summary assignments (as defined in
 %%     Section~\ref{sec:interproc}). Then for any vertex $v$,
 %%     \[ \sound{\mathscr{I}\tuple{v}}{\mathscr{J}\tuple{v}} \]

 %%     Moreover, this holds even if $\mathcal{I}$ and $\mathcal{J}$ do not
 %%     satisfy any of the \QPKA{} axioms.
 %%   \end{lemma}
 %%   \begin{proof}
 %%     This is essentially a corollary of Lemma~\ref{lem:pathexp_rel}.  Recall
 %%     that
 %%     \[ \mathscr{I}\tuple{v} = \mathscr{I}(\overline{S}_{\mathcal{I}})[\pathexp{P_1}{P_k}] \mul_\mathcal{I} \mathscr{I}(\overline{S}_{\mathcal{I}})[\pathexp{\entry_k}{v}] \]
 %%     \[ \mathscr{J}\tuple{v} = \mathscr{J}(\overline{S}_{\mathcal{J}})[\pathexp{P_1}{P_k}] \mul_\mathcal{J} \mathscr{J}(\overline{S}_{\mathcal{J}})[\pathexp{\entry_k}{v}] \]
 %%   So we need only to prove that
 %%   \[ \sound{\mathscr{I}(\overline{S}_{\mathcal{I}})[\pathexp{P_1}{P_k}]}{\mathscr{J}(\overline{S}_{\mathcal{J}})[\pathexp{P_1}{P_k}]} \]
 %%   and 
 %%   \[ \sound{\mathscr{I}(\overline{S}_{\mathcal{I}})[\pathexp{\entry_k}{v}]}{\mathscr{J}(\overline{S}_{\mathcal{J}})[\pathexp{\entry_k}{v}]} \]
 %%   The latter follows directly from Lemma~\ref{lem:pathexp_rel}.  It remains
 %%   to show the former.

 %%   Recall that the interpretation of a call graph edge $P_i \rightarrow P_j$
 %%   is defined in terms of the interpretations of the path expression
 %%   $\pathexp{\entry_i}{c}$ describing paths to a vertex $c$ that calls $j$.
 %%   It follows from Lemma~\ref{lem:pathexp_rel} that we must have
 %%   \[ \sound{\mathscr{I}(\overline{S}_{\mathcal{I}})[P_i \rightarrow P_j]}{\mathscr{J}(\overline{S}_{\mathcal{J}})[P_i \rightarrow P_j]} \]
 %%   for all edges $P_i \rightarrow P_j$ in the call graph.  We may then prove by
 %%   induction on $\pathexp{P_1}{P_k}$ that
 %%   \[ \sound{\mathscr{I}(\overline{S}_{\mathcal{I}})[\pathexp{P_1}{P_k}]}{\mathscr{J}(\overline{S}_{\mathcal{J}})[\pathexp{P_1}{P_k}]} \]
 %%   \end{proof}
 %%   We can prove that for all $i$,
 %%   $\sound{\overline{S}_{\mathcal{C}}(i)}{\overline{S}_\mathcal{A}(i)}$ in the
 %%   standard way, by induction on the transfinite iteration sequence defining
 %%   $\overline{S}_{\mathcal{C}}$ (using Lemma~\ref{lem:pathexp_rel} for the
 %%   induction step).  We then have the main result by applying
 %%   Lemma~\ref{lem:analysis_rel}.
 %% \end{proof}


 %% \subsection{Galois connections} \label{sec:interproc_galois}
 %% It is straightforward to adapt the Galois connection framework to the
 %% interprocedural case: all that is needed is an additional condition that
 %% abstract quantification operator approximates the concrete quantification
 %% operator.  Formally, we have the following theorem:
 %% \begin{theorem}
 %%   Let $\mathscr{C}, \mathscr{A}$ be interpretations over complete \QKA{}s,
 %%   and let $\mathcal{C} \galois{\alpha}{\gamma} \mathcal{A}$ be a Galois
 %%   connection such that
 %%   \begin{itemize}

 %%   \item $a \absmul a' \absgeq \alpha(\gamma(a) \natmul \gamma(a'))$
 %%   \item $a^\absstar \absgeq \alpha(\gamma(a)^\natstar)$
 %%   \item $1_{\mathcal{A}} \absgeq \alpha(1_{\mathcal{C}})$
 %%   \item $\exists_{\mathcal{A}} x. a \absgeq \alpha(\exists_{\mathcal{C}} x. \gamma(a))$
 %%   \end{itemize}
 %%   Then for any vertex $v$, $\alpha(\mathscr{C}\langle v \rangle) \absleq
 %%   \mathscr{A}\langle v \rangle$.
 %% \end{theorem}
 %% %% \begin{proof}
 %% %%   As in Theorem~\ref{thm:sound_abstraction}, except we use the fixpoint
 %% %%   transfer theorem to establish the approximation of
 %% %%   $\overline{S}_{\mathcal{C}}$ by $\overline{S}_{\mathcal{A}}$.
 %% %% \end{proof}

 %% \begin{example}[Reaching definitions]
 %%   Recall that an element of the abstract domain for reaching definitions is a
 %%   pair $\langle d, v \rangle$ consisting of a set of definitions $d$ that may
 %%   be generating along a path and a set of variables $v$ that must be killed
 %%   along any path.  We define existential quantification on this domain as
 %%   follows:
 %%   \[ \exists^{\mathscr{D}} x. \langle d,v \rangle = \langle \{ e \in d : D(e) \neq \{x\} \}, v\setminus \{x\} \rangle \]

 %%   Thus, moving the variable $x$ out of scope in reaching definitions analysis
 %%   ``forgets'' the reaching definitions of $x$ and removes $x$ from the set of
 %%   variables that must be killed.  This ensures that reaching definitions of a
 %%   local variable cannot ``leak'' from a called procedure back to its calling
 %%   context, and that procedures cannot kill the definition of a local
 %%   variable.
 %% \end{example}

